Formal Analysis of Lending Pools in Decentralized Finance

Decentralised Finance (DeFi) applications constitute an entire financial ecosystem deployed on blockchains. Such applications are based on complex protocols and incentive mechanisms whose financial safety is hard to determine. Besides, their adoption is rapidly growing, hence imperilling an increasingly higher amount of assets. Therefore, accurate formalisation and verification of DeFi applications is essential to assess their safety. We have developed a tool for the formal analysis of one of the most widespread DeFi applications: Lending Pools (LP). This was achieved by leveraging an existing formal model for LPs, the Maude verification environment and the MultiVeStA statistical analyser. The tool supports several analyses including reachability analysis, LTL model checking and statistical model checking. In this paper we show how the tool can be used to analyse several parameters of LPs that are fundamental to assess and predict their behaviour. In particular, we use statistical analysis to search for threshold and reward parameters that minimize the risk of unrecoverable loans.

==> Chapters/3-exec_model.tex <==
\ChapSec{A Maude specification of Lending Pools}
\label{chap:lp-model}

This chapter discusses a Maude specification of the lending pools model presented in \Cref{subsec:lp}. This specification will allow to automatically simulate the LP rules on arbitrary configurations. Subsequently, in \Cref{chap:agents}, this development will be extended in order to conduct statistical analysis on LP.

% introduce what each section is about
Specifically, \Cref{sec:impl} describes the basic types required to model LP configurations. \Cref{sec:rules} outlines the implementation of the model rules. Finally, \Cref{sec:overall-dev} discusses the language features used for the model parameterisation and testing.

% \todo[inline]{Create public repo \texttt{maude-lp} with spec only, under GPLv2 guide \href{https://www.gnu.org/licenses/old-licenses/gpl-2.0.html\#SEC4}{here}. \\ NOTE: MV is not GPL then don't share MV integration!}

As reminded in each listing throughout this chapter, \Cref{chapter:app-maude} contains the essential modules of the developed specification. The full specification is open source, under the GNU General Public License version 2 at \cite{mirelli2021maudelp}.

% Figuratively, the model itself could be considered to be a language. In that case, \Cref{sec:impl,sec:rules} are to be viewed as an introduction to respectively the language syntax and semantics.

\SecSubSec{The model basic components}
\label{sec:impl}

This section describes the Maude modules developed in order to represent the basic components of an LP configuration. \Cref{subsec:toks} overviews the tokens type system and introduces the abstraction implementing mathematical functions. \Cref{subsec:pools} exemplifies the usage of such abstraction, defining an essential component of an LP configuration: a pool.

\SSecSSSec{Tokens}
\label{subsec:toks}

The model formalised by Bartoletti et al.\,\cite{bartoletti2020sok} heavily relies on basic mathematical concepts including sets and functions, mainly in order to formalise the mechanisms used for transferring tokens among parties. Consequently, the tokens abstraction is used by this section to explain how these mathematical means, namely sets and functions, have been defined in Maude. In order to achieve this, the section discusses how the following concepts, defined in \Cref{subsec:lp}, have been specified:

\begin{enumerate}
\item the basic token types, minted and free tokens;
\item the sets of token types, $T_{f} \subseteq \FTokens$ and $T_{m} \subseteq \MTokens$;
\item the functions from token types to non-negative real numbers, $\WalletOf{\Agent{A}}$, for agent $\Agent{A}$.
\end{enumerate}

Distinguishing between free and minted tokens is essential in order to specify LP. Precisely, it is desirable to model $\tau_{i}\ \mathrm{and}\ \tau_{i}'\ \forall\ i \in \mathbb{N}$ as respectively free and minted tokens. \Cref{lst:mf-tok} shows how this is obtained in Maude. For instance, the operators \texttt{tau(\_)} and \texttt{\_'}, in \Cref{mf-def3,mf-def4}, allow to specify $\tau_{0}$ with the term \texttt{tau(0)} and $\tau_{0}'$ with \texttt{tau(0)'}, respectively of sort \texttt{Free-Token} and \texttt{Minted-Token}. Notably, free and minted tokens are defined as subsorts, \texttt{Free-Token}, \texttt{Minted-Token}, of \texttt{Token} (\Cref{mf-def1,mf-def2}). 

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=\MListFrm\baselineskip]
  \begin{lstlisting}[
    style=maude-snippet-style,    
    label=lst:mf-tok,
    caption={Maude definition of \texttt{Free-Token} and \texttt{Minted-Token}, extract from \Cref{lst:tokens-full}, \Cref{lst-ln:tokens} }
    ]
fmod TOKENS is ---[\CodeLineBreak]
    sort Token Free-Token Minted-Token . ---[\label{mf-def1}]
    subsort Minted-Token Free-Token < Token . ---[\label{mf-def2} \CodeLineBreak]
    op tau(_) : Nat -> Free-Token [ctor ...] . ---[\label{mf-def3}]
    op _' : Free-Token -> Minted-Token [ctor ...] . ---[\label{mf-def4} \CodeLineBreak] 
endfm
  \end{lstlisting}
\end{mdframed}


In order to manage several free and minted tokens, two types for sets of token types have been developed: \texttt{Set\{Free-Token\}} and \texttt{Set\{Minted-Token\}}. For example, the two types allow to specify the set of free tokens $\{\tau_{0}, \tau_{1}, \tau_{2}\}$ as the term \mbox{\texttt{tau(0), tau(1), tau(2)}} of sort \texttt{Set\{Free-Token\}}. Conversely, the set of minted tokens $\{\tau_{0}', \tau_{1}', \tau_{2}'\}$ is expressible as the term \texttt{tau(0)',\,tau(1)', tau(2)'} of sort \texttt{Set\{Minted-Token\}}. The parametric module \texttt{SET\{X::TRIV\}}\footnote{The parameterised module \texttt{SET\{X::TRIV\}} and the view \texttt{TRIV} are defined in \Cref{lst:set-def,lst:triv-def}, respectively.} is used to implement \texttt{Set\{Free-Token\}} and \texttt{Set\{Minted-Token\}}, representing free and minted tokens sets, respectively. Similarly to the relation we have observed in \Cref{lst:mf-tok}, also \texttt{Set\{Free-Token\}} and \texttt{Set\{Minted-Token\}} are defined as subsorts of  \texttt{Set\{Token\}}. This is achieved by the parameterised module \texttt{SUBSET\{X::TRIV,\,Y::TRIV\}}\footnote{\Cref{lst:abs-full}, \Cref{cod:def-sset}.} in \Cref{lst:tokens-full}, \Cref{lst-ln:decl-sset}, which allows to define "mixed" token type sets such as $\{\tau_0, \tau_1, \tau_1'\}$ as \texttt{tau(0),tau(1), tau(1)':Set\{Token\}}.

Functions are the last abstraction which serves to model essential LP objects, including agents' wallets, $\pi_{f}, \pi_{m}\ \mathrm{and}\ \pi_{l}$. Consequently, it is desirable to define functions, as per their usual mathematical definition\footnote{A function $f$ of domain $D$ and codomain $C$, denoted as $f: D \rightarrow C$, is defined as $f \subseteq D \times C\ \mathrm{and}\ \forall c \in\ C\ \exists!\ d \in D\ .\ (d, c) \in f$. \iffalse as a set of ordered pairs $(d,c)$ s.t.\,$d \in D, c \in C$ and $\forall d \in D \ \exists ! \ c \in C$.\fi }, in a parametric manner. In this sense, the sorts \texttt{Map\{X,Y\}}, \texttt{Set\{X\}} and \texttt{Set\{Y\}} are employed: \texttt{Map\{X,Y\}} can be used to store the pairs composing a function, as shown in \Cref{subsec:fmod}, while \texttt{Set\{X\}} and \texttt{Set\{Y\}}  for the definition of the operators computing the function domain and codomain. \Cref{lst:fun} shows the approach used to define a generic function offering the operations for determining its domain (\texttt{dom}) and codomain (\texttt{cod}\footnote{For brevity, only the implementation of \texttt{dom} is illustrated, as \texttt{cod} is analogous.}). Notably, the \texttt{FUNCTION} module is parameterised with respect to a \texttt{MAP-THEORY}, \texttt{MT}, acting as the entity binding \texttt{Map\{X,Y\}} with the sorts corresponding to its domain (\texttt{Set\{X\}}) and codomain (\texttt{Set\{Y\}}). The operator \texttt{dom} is defined via the operator \texttt{\$dom} which utilises all the sorts and operators of \texttt{MT}, in order to produce a set of \texttt{MT\$D}-sorted terms. \Cref{lst:map-th} illustrates the sorts and operators of a \texttt{MAP-THEORY}, described below.

\begin{itemize}
\item [\texttt{E}, \texttt{M} - ] represent respectively an \texttt{Entry\{X,Y\}} and a \texttt{Map\{X,Y\}};
\item [\texttt{D}, \texttt{DT} - ] define the domain type (in the form of \texttt{Set\{X\}}) and its elements' type (\texttt{X});
\item [\texttt{C}, \texttt{CT} - ] model the codomain type (in the form of \texttt{Set\{Y\}}) and its elements' type (\texttt{Y}).
\end{itemize}

Similarly, the operators in \texttt{MAP-THEORY} are defined as the main operators in \texttt{MAP\{X::TRIV,Y::TRIV\}} and \texttt{SET\{X::TRIV\}}, as further explained.

\begin{itemize}
\item [\texttt{\_|->\_} - ] is syntactically equivalent to the constructor for a term of sort \texttt{Entry\{X,Y\}}, \texttt{\_|->\_}, \Cref{lst:map-def} \Cref{lst-ln:ops-def1}. 
\item [\texttt{\_;\_}   - ] is syntactically equivalent to the constructor for a term of sort \texttt{[Map\{X,Y\}]}, \texttt{\_;\_}, \Cref{lst:map-def} \Cref{lst-ln:ops-def2}. 
\item [\texttt{\_,\_}   - ] is syntactically equivalent to the constructor of non-empty \texttt{Set\{X\}} in \Cref{lst:set-def} \Cref{lst-ln:set-op}.
\end{itemize}

% In the case of \texttt{E}, \texttt{M} ( and \texttt{\_;\_}) have the same form as the ones defined in the \texttt{MAP\{X,Y\}} module for modelling respectively a single \texttt{Entry} and a \texttt{Map} (or \texttt{\_;\_}-composition of \texttt{Entr}ies). Conversely, the signature of the remaining operators (\texttt{\_,\_}) coincide with the constructor of a \texttt{NeSet}\footnote{As defined in \texttt{SET\{X::TRIV\}} and documented in \cite{clavel2020maude}, Section 7.13.2.}.

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=\MListFrm\baselineskip]
  \begin{lstlisting}[
    style=maude-snippet-style,    
    label=lst:fun,
    caption={Maude definition of the \texttt{FUNCTION} main functionalities: \texttt{dom} and \texttt{cod}, extract from \Cref{lst:abs-full}, \Cref{lst-ln:func} }
    ]
fmod FUNCTION{MT :: MAP-THEORY} is
    var map : MT$M .  ---[\label{lst-ln:MT-M}]
    var domElt : MT$DT .
    var codElt : MT$CT .
    var domSet : MT$D .
    var codSet : MT$C .

    --- dom implements the function domain as a set
    --- of MT$D-sorted terms    
    op dom : MT$M -> MT$D .
    eq dom(map) = $dom(map, emptyD) .

    --- $dom is dom auxilary function, implementing
    --- the actual logic to iterate over the map and
    --- extract its values
    op $dom : MT$M MT$D -> MT$D . 
    eq $dom((map ; domElt |-> codElt), domSet) = 
                             $dom(map, (domSet, domElt)) .
    eq $dom((domElt |-> codElt), domSet) = domSet, domElt .
    eq $dom(emptyM, domSet) = domSet .

    --- cod implements the function codomain as a set
    --- of MT$C-sorted terms
    op cod : MT$M -> MT$C .---[\CodeLineBreak]
endfm
    ---[%$]
  \end{lstlisting}
\end{mdframed}

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=\MListFrm\baselineskip]
  \begin{lstlisting}[
    style=maude-snippet-style,    
    label=lst:map-th,
    caption={Maude definition of \texttt{MAP-THEORY}, binding \texttt{Map\{X,Y\}} with \texttt{Set\{X\}} and \texttt{Set\{Y\}}, extract from \Cref{lst:abs-full}, \Cref{lst-ln:map-th}}
    ]
fth MAP-THEORY is 
    sorts M E DT CT D C .

    --- entry (pair) is subsort of map (set of pairs)
    subsort E < M .
    --- constructing the map pairs
    op _|->_ : DT CT -> E [ctor] .
    --- `assoc` and `comm` make map pairs unordered
    op _;_ : [M] E -> [M] [ctor id: emptyM assoc comm prec
                           121 format (d r os d)] .
    --- empty pair
    op emptyM : -> M .

    --- CT is the sort of the terms in Set{C}     
    subsort CT < C .
    --- DT is the sort of the terms in Set{D}     
    subsort DT < D .
    
    --- operator to be bound to (empty).Set{C}
    op emptyC : -> C .
    --- operator to be bound to (_,_).Set{C}
    op _,_ : C CT -> C
    [ctor assoc comm prec 121 format (d r os d)] .

    --- operator to be bound to (empty).Set{D}
    op emptyD : -> D .
    --- operator to be bound to (_,_).Set{D}
    op _,_ : D DT -> D
    [ctor assoc comm prec 121 format (d r os d)] .
endfth    
  \end{lstlisting}
\end{mdframed}

As exemplified in \Cref{subsec:pools}, this approach allows the modeller to instantiate a function by reusing the logic in \Cref{lst:fun} to compute its domain and codomain, by module parameterisation\footnote{\Cref{subsec:param-modules} outlines Maude parametric programming.}. This is achieved following the procedure\footnote{More extensively described in \cite{clavel2020maude}, Section 6.3.4.}:

\begin{enumerate}
\item defining a generic module \texttt{<FUN-MOD>} containing the sorts and operators to be bound to \texttt{MAP-THEORY} ones;
\item producing a generic view \texttt{<FUN-VIEW>} binding \texttt{<FUN-MOD>} to \texttt{MAP-THEORY};
\item instantiating the function by \texttt{including FUNCTION\{<FUN-VIEW>\} .}
\end{enumerate}

As a result, the module importing \texttt{FUNCTION\{<FUN-VIEW>\}} is equipped with sort \texttt{Map\{X,Y\}} and the operators \texttt{dom} and \texttt{cod} returning respectively a \texttt{Set\{X\}}-typed domain and a \texttt{Set\{Y\}}-typed codomain.

\SSecSSSec{Pools}
\label{subsec:pools}

The Maude implementation of a pool, $\pi$, defined in \Cref{subsec:lp}, is based on \texttt{FUNCTION\{MT::MAP-THEORY\}}, as shown in \Cref{fig:pi-hier}. The figure depicts the modules imported in \texttt{LP}, which implement the main functionalities of $\pi$. The pool components (functions $\pi_{f}$, $\pi_{l}$ and $\pi_{m}$) are modelled via \texttt{FUNCTION\{MT\}} and instantiated by means of the views \texttt{PiFFun}, \texttt{PiLFun} and \texttt{PiMFun} binding the specific \texttt{FUNCTION\{MT\}} operators and sorts to \texttt{MAP-THEORY} ones. The remaining included module, namely \texttt{WALLET}, defines basic operations on wallets which are useful to specify $\pi$.

\begin{figure}
  \centering
  \includegraphics[width=.8\linewidth]{../figures/pi-hier.png}
  \caption{Importation graph of the \texttt{LP} functional module}
  \label{fig:pi-hier}
\end{figure}

In order to clarify the usage of \texttt{FUNCTION}, the rest of the section describes \texttt{PI-FUND}, the module containing the specification for $\pi_{f}$\footnote{\texttt{PI-LOAN} and \texttt{PI-MINT} are developed similarly so to model the remaining pool components: $\pi_{l}$ and $\pi_{m}$.}. \Cref{lst:pi-fund} illustrates how to instantiate \texttt{FUNCTION\{MT\}} by the view \texttt{PiFFun}. 

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=\MListFrm\baselineskip]
  \begin{lstlisting}[
    style=maude-snippet-style,    
    label=lst:pi-fund,
    caption={Maude definition of \texttt{PI-FUND}, extract from \Cref{lst:pools-full}, \Cref{lst-ln:pi-fund}}
    ]
fmod PI-FUND is
    protecting FUNCTION{PiFFun} . ---[\CodeLineBreak]
endfm    
  \end{lstlisting}
\end{mdframed}

\Cref{lst:pi-f} fully specifies the way the binding, operated by the view, is achieved. Specifically, the \texttt{Map} underlying $\pi_{f}$\footnote{Defined in the original formal model as a function mapping a free token type to a rational number.} (\texttt{MT\$M}, in \texttt{FUNCTION\{M\}}, \Cref{lst:abs-full}, \Cref{lst-ln:MT-M}) is a \texttt{Map} from a \texttt{Token} to a \texttt{Float0+}\footnote{A real non-negative number.}. As a result, the basic sorts for domain and codomain elements, \texttt{DT} and \texttt{CT}, are bound to \texttt{Token} and \texttt{Float0+}. Similarly, the domain and codomain sorts, \texttt{D} and \texttt{C}, are bound to \texttt{Set\{Token\}} and \texttt{Set\{Float0+\}}, respectively. Additionally, it is worth observing that \texttt{FUNCTION\{PiFFun\}} not only offers the means to model wallets\footnote{As defined in \Cref{subsec:lp}.}, but it is also fundamental for defining  \texttt{FUNCTION\{PiLFun\}}\footnote{Note that its codomain can be modelled as a \texttt{Map\{Token, Float0+\}}.} and  \texttt{FUNCTION\{PiMFun\}}. In fact, as shown in \Cref{fig:pi-hier}, \texttt{FUNCTION\{PiFFun\}} is included in \texttt{SUBTOKEN-FUNCTIONS}, the module representing the sorts and operators bound by \texttt{PiLFun} and \texttt{PiMFun}.

%\Footnote{\texttt{Agent-Id} is the sort used to specify the \texttt{Agent} type in \cite{bartoletti2020sok}. The sort \texttt{Agent} will be introduced in \Cref{chap:agents}.}

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=\MListFrm\baselineskip]
  \begin{lstlisting}[
    style=maude-snippet-style,    
    label=lst:pi-f,
    caption={Maude definition of \texttt{PiFFun}, the view binding \texttt{MAP-THEORY} to the sorts and operators specifying $\pi_{f}$, extract from \Cref{lst:pools-full}, \Cref{lst-ln:pi-f} }
    ]
view PiFFun from MAP-THEORY
                 to TOKEN-MAP is
    sort M to Map{Token, Float0+} .
    sort E to Entry{Token, Float0+} .

    sort DT to Token .
    sort CT to Float0+ .

    sort D to Set{Token} .
    sort C to Set{Float0+} .

    op emptyD to empty .
    op emptyC to empty .
endv
\end{lstlisting}
\end{mdframed}

\SecSubSec{LP rules}
\label{sec:rules}

This chapter draws the attention on specification of the LP actions in Maude. First, \Cref{subsec:config-obs} defines the LP configurations modelled in Maude. Second, \Cref{subsec:act-to-rule} examines the semantics of the object-based approach and motivates the main changes to the initial model notation. 

\SSecSSSec{Configurations definition}
\label{subsec:config-obs}

\Cref{lst:gamma} expresses an example of a simple LP configuration in Maude.

\begin{mdframed}[style=codeframe-style]
  \begin{lstlisting}[
    style=maude-syntax-def-style,    
    label=lst:gamma,
    caption={Maude definition of a simple LP configuration}
    ]
[
  Pi | p 
  (< A : noState | * sigma_A >
   < B : noState | * sigma_B >
   < C : noState | * sigma_C >)
   < R(n) : Round | none >
   < P(0) : LiqParams | CMin(cminV), 
                        Rliq(rliqV) >
] :: ClosedConfiguration
\end{lstlisting}
\end{mdframed}

The Maude representation of a (\texttt{Message}-less\footnote{\Cref{subsec:act-to-rule} discusses LP configuration holding messages.}) LP configuration comprises nearly the same components, as discussed in \Cref{subsec:lp}. Firstly, \texttt{Pi | p} is a term of sort \texttt{BC\{LP\}}, defined as an \texttt{Object} in \Cref{lst:configuration-full}, \Cref{lst-ln:bc-lp}. The term \texttt{pi} models the pool $\Pool$ state. Conversely, \texttt{p} models the assets price function, $\Price$, via a simple \texttt{Map\{Token, Float0+\}}. Secondly, a generic object of the form \mbox{\texttt{< Id : noState | * sigma\_Id >}} represents an agent identified by \texttt{Id}, having a \texttt{noState} behaviour\footnote{\Cref{chap:agents} details a specific behaviour type.} and holding a wallet \texttt{sigma\_Id}\footnote{Wallet of agent identified by $\Agent{Id}$, $\WalletOf{\Agent{Id}}$ in \Cref{subsec:pools}.}. Thirdly, the term \mbox{\texttt{< R(n) : Round | none >}} is an \texttt{Object} added to the configuration in order to store the \texttt{n}-th blockchain round. Finally, \texttt{< P(0) : LiqParams | CMin(cminV), Rliq(rliqV) >} is employed to parameterise the configuration given by \texttt{CMin} (\texttt{cminV}) and \texttt{Rliq}\footnote{Namely, $\CMin\ \mathrm{and}\ \Rliq$.}. (\texttt{rliqV}) parameters, as shown in \Cref{subsec:model-feat}. Additionally, it is worth noting that the sort of a LP configuration term is \texttt{ClosedConfiguration}. A \texttt{ClosedConfiguration} is obtained from a \texttt{Configuration} by the operator \texttt{[\_] : Configuration -> ClosedConfiguration}, as shown in \Cref{lst:gamma}. As \Cref{subsec:act-to-rule} shows, this is a fundamental operator in order to modify only specific components of a \texttt{Configuration}, while maintaining the rest intact.

The full implementation of LP configuration is contained in \texttt{BC-LP-CONFIGURATION}, whose main dependencies are pictured in \Cref{fig:lp-config}. Specifically, \texttt{BC\{LP\}} contains the sorts and operators discussed in \Cref{subsec:pools}, whereas \texttt{CONFIGURATION} is the essential system module explained in \Cref{subsec:mod}. Next, \texttt{AGENT-STATE} and \texttt{BC-LP-CONFIG-COMPONENTS} define additional syntactic sugar, mainly destructuring operators, which allow to decompose a \texttt{Configuration} into its atomic components. Lastly, \texttt{LP-PARAMETERS} defines the lending pools essential parameters discussed in \Cref{subsec:model-feat}.

\begin{figure}
  \centering
  \includegraphics[width=.6\linewidth]{../figures/lp-config.png}
  \caption{Importation graph of the \texttt{BC-LP-CONFIGURATION} system module}
  \label{fig:lp-config}
\end{figure}

\SSecSSSec{Translating LP actions into Maude rules}
\label{subsec:act-to-rule}

% 1. Talk about how the LP actions were converted into rules
% However, the factual translation of LP actions could not be achieved without the fundamental object abstraction introduced in \Cref{subsec:config-obs}.

As stated in \Cref{subsec:config-obs}, the objects abstraction is essential for defining LP actions. Specifically, \texttt{Object}s (in case of lending pools, the agents and the pool) need to interact with one another by means of \texttt{Message}s. In these specifications, LP actions are syntactically modelled as \texttt{Message}s, whereas their semantics are specified by the rewriting rules consuming those \texttt{Message}s. As a result, the LP rule $\mathrm{r_{\Agent{A}}}(z^{n})$ of a given arity $n$ is syntactically defined as the Maude operator in \Cref{lst:act-to-rule}.

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=\MListFrm\baselineskip]
  \begin{lstlisting}[
    style=maude-syntax-def-style,    
    label=lst:act-to-rule,
    caption={Syntax of a message representing an issued LP actions in Maude.}
    ]
op r : Agent-Id S1... Sn -> Message .    
\end{lstlisting}
\end{mdframed}

In the listing, \texttt{S1}...\texttt{Sn} are the sorts of the terms \texttt{t1}...\texttt{tn} representing the $n$ input parameters $z^{n}$. Contrarily, the first input parameter of the operator \texttt{r} is a term \texttt{A:Agent-Id}, identifying the agent issuing the message. Consequently, the action $\mathrm{r_{A}}(z^{n})$ is represented in Maude by \texttt{r(A, t1, ..., tn):Message}.

However, actions cannot be implemented as mere syntactic constructs, since they directly imply a system state change, whose semantics ought to be defined. This is exactly the purpose of the rewriting rules subsequently discussed. Specifically, conditional rewriting rules, following the syntax in \Cref{lst:action-syntax}, are used to model LP actions semantics.

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=\MListFrm\baselineskip]
  \begin{lstlisting}[
    style=maude-syntax-def-style,    
    label=lst:action-syntax,
    caption={A generic Maude rewrite rule expressing the semantics of an LP action.}
    ]
crl [r-id] :
    [ gamma r(A:Agent-Id, t1:S1, ..., tn:Sn) ]
                                               => [ gamma' ]
          if G(gamma, A, t1, ..., tn) .
\end{lstlisting}
\end{mdframed}

Here, \texttt{[r-id]} is the rule identifier, mainly used for debugging purposes, whereas \texttt{gamma} and \texttt{gamma'} are terms of sort \texttt{Configuration}, representing respectively the system state before\footnote{Modulo \texttt{r(A, t1, ..., tn).}} and after the rewrite occurs. Next, \texttt{r(A, t1, ..., tn)} is the message whose consumption entails the transition from state \texttt{gamma} to \texttt{gamma'} according to the semantics expressed by \texttt{gamma'} and \texttt{G(gamma, A, t1, ..., tn)}. Lastly, \texttt{G(gamma, A, t1, ..., tn)} (also named a guard) is a proposition, which given the left-hand side terms, allows the rule to be executed only if it is evaluated to true. Thus, intuitively, the aforementioned rule can be executed in a state \texttt{[ gamma0 ]} if and only if \texttt{gamma0} contains \texttt{r(A, t1, ..., tn):Message}\footnote{For some \texttt{A, t1, ..., tn} terms of sorts \texttt{Agent-Id, S0, ..., Sn}} and \texttt{G(gamma0, A, t1, ..., tn)} is true. Noteworthily, the implementation choice of the \texttt{ClosedConfiguration} constructor (\texttt{[\_]}) is essential to match the unmodified \texttt{Object}s of \texttt{gamma0} against the rule left-hand side.

% Resultantly, lending pools actions can be naturally expressed through the use of Maude rewrite rules. More generally, this is also a consequence of the fact that LP rules can be formulated by Horn clauses, translatable, in Maude, into rewriting rules and equations.

% 2. Add a rule example here -> liquidate
As a result, a rewriting rule implementing the LP action $\mathrm{r}_{\Agent{A}}(z^{n})$ induces the consumption of the message \texttt{r(A, t1, ..., tn)}. Clearly, the rewrite application yields changes to the initial configuration according to the semantics of the LP action. The rest of this section exemplifies this point, by describing the liquidate LP action $\mathrm{Liq}_{\Agent{A}}(\Agent{B}, v: \hat{\tau}, \tau')$, as defined in \Cref{fig:liquidate-rl}.

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=-4.8\baselineskip]
  \begin{lstlisting}[
    style=maude-snippet-style,    
    label=lst:liquidate,
    caption={Definition of $\mathrm{Liq}_{\Agent{A}}(\Agent{B}, v: \hat{\tau}, \tau')$ in Maude, simplified extract from \Cref{lst:configuration-full}, \Cref{lst-ln:liquidate}. Apart from the removed rules, the only modification to the appendix is the renaming of \texttt{tau} in \texttt{hTau}. This is to align the notation with \Cref{fig:liquidate-rl}.}
    ]
crl [liquidate] :          --- i. represents the i-th
   [ gamma                 --- constraint in the liquidate
   < R(r) : Round | none > --- action def (Figure 2.1)
   < A : agState | * sigmaA >
   < B : agState' | * sigmaB >
   (pi | p) 
   liquidate(A, B, (v, hTau), tau') ]
   => [ gamma
      < R(r + 1) : Round | none >
      < A : agState | * sigmaA' > 
      < B : agState' | * sigmaB' > 
      (pi' | p) ]
   if v' := v * (p[hTau] / (p[(pi).u(tau')])) *     --- 4.
                                   (gamma).Rliq /\ ---[\label{lst-ln:destr-example-rliq}]
      sigmaA' := (sigmaA - v : hTau) + v' : tau' /\ --- 8.
      sigmaB' := sigmaB - v' : tau' /\              --- 9.
      (gamma  < A : agState | * sigmaA > 
              < B : agState' | * sigmaB > 
              (pi | p) ).C(B) < (gamma).CMin /\    --- 10. ---[\label{lst-ln:destr-example-cmin}]
      gamma' := gamma                    --- final config
            < A : agState | * sigmaA' >  --- after rule
            < B : agState' | * sigmaB' > --- application
            (pi' | p) /\
      (gamma').C(B) <= (gamma).CMin .              --- 11.
\end{lstlisting}
\end{mdframed}

In the liquidate rule, the left-hand side matches (i.e.\,it can be applied to) any configuration containing a liquidate message involving two existing users and satisfying the rule condition. The condition is a simplification of the original, showing the action semantics of the essential constraints\footnote{The preconditions \LiqC{4}, \LiqC{8}, \LiqC{9}, \LiqC{10} and \LiqC{11} in \Cref{fig:liquidate-rl}.} detailed in \Cref{subsec:lp}. Initially, it should be noted that only the components destructured from the left-hand side \texttt{Configuration} are modified by the action: liquidator (\texttt{A}) and borrower (\texttt{B}) agents\footnote{Henceforth, agent \texttt{Object}s will be referred to by their id term of sort \texttt{Oid}.}, blockchain round object and \texttt{(pi | p)}. Obviously, the input terms to the liquidate message\footnote{\texttt{A, B, (v, hTau), tau'}} are utilised as well. Subsequently, the rule condition shows how these parameters are used, explaining the exact action behaviour. First, matching equation having \texttt{v'} as the left-hand side assigns to \texttt{v'} the units of \texttt{tau'}, i.e.\,the amount of the liquidation seized collateral. Second, the liquidator and borrower's initial balances are updated reflecting the fact that the liquidator repays \texttt{v} units of \texttt{hTau} (borrower's loan) in return for \texttt{v'} units of \texttt{tau'}. Third, it is verified that the collateralization of \texttt{B} in the left-hand side configuration is below \texttt{CMin}\footnote{The configuration destructors of \texttt{CMin} (\texttt{(gamma).CMin}) and of the other LP parameters are discussed in \Cref{subsec:model-feat}.}. Lastly, the final \texttt{ClosedConfiguration} (\texttt{gamma'}) is reconstructed from the updated objects\footnote{Namely \texttt{A}, \texttt{B} and \texttt{pi'}, whose update is not shown in \Cref{lst:liquidate}} and \texttt{B}'s collateralization, based on \texttt{gamma'}, is compared to \texttt{CMin}. Thus, the condition is satisfied, i.e.\,the rule is executable, if and only if the borrower's collateralization is less or equal than \texttt{CMin}, after the action has been executed\footnote{I.e.\,when the system is in state \texttt{gamma'}.}.

\SecSubSec{The model specifications}
\label{sec:overall-dev}

This section summarises the current specifications development, underlining two particularly desirable properties expected from any high-quality piece of software: parameterization capability and testability. Specifically, \Cref{subsec:model-feat} discusses the parameters which could be used to instantiate an LP configuration, whereas \Cref{subsec:test} focusses on the Maude features employed for testing the specifications.

\SSecSSSec{The model parameterization}
\label{subsec:model-feat}
% discuss what has been implemented in terms of:
% 1. configuration observers (value functions + collateralization)
% 2. model actions
% 3. model parameters module

The lending pools model ought to have a number of parameters in order to offer a more realistic representation of the underlying financial platforms. Consequently, the Maude specification of LP should expose functionalities in order to set and modify those parameters. The model can be instantiated by choosing at least three parameters ($\CMin$, $\Rliq$ and $\Maxliq$), introduced in \Cref{subsec:lp}. The respective terms specifying them in Maude are presented below.

\begin{itemize}
  \item [\texttt{CMin}] - the threshold indicating the minimum collateralization a user may have without risking to be liquidated. It models $\CMin$.
  \item [\texttt{Rliq}] - the discount rate applied to the amount of tokens seized by the liquidator during a liquidation. It models $\Rliq$.
  \item [\texttt{Maxliq}] - threshold expressing the maximum amount of repayable loan during a single liquidation. It models $\Maxliq$.
\end{itemize}

These parameters are defined in \texttt{LP-PARAMETERS}\footnote{\Cref{lst:configuration-full}, \Cref{lst-ln:params}}, and the value of \texttt{CMin} and \texttt{Rliq} can be modified via the operator \texttt{replaceLiqParams}, in \Cref{lst:rep-liq-params} \Cref{lst-ln:repLiqP}. Notably, the operator either inserts a new \texttt{Object} of class \texttt{LiqParams}\footnote{As shown in \Cref{lst:gamma}} (\Cref{lst-ln:liqParams-add}) or it updates the current \texttt{CMin} and \texttt{Rliq} values (\Cref{lst-ln:liqParams-upd}). Therefore, reducing the term \texttt{(gamma).replaceLiqParams(1.5, 1.1)} determines that \texttt{CMin} is set to \texttt{1.5} and \texttt{Rliq} to \texttt{1.1}. The new values are then accessed through \texttt{gamma}'s destructors defined in \Cref{lst:liq-params-destr}. Examples of their usage can be observed in \Cref{lst:liquidate} \Cref{lst-ln:destr-example-rliq,lst-ln:destr-example-cmin} for \texttt{Rliq} and \texttt{CMin}, correspondingly.

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=\DTUMListFrm\baselineskip]
  \begin{lstlisting}[
    style=maude-snippet-style,    
    label=lst:rep-liq-params,
    caption={Maude definition of the operator \texttt{replaceLiqParams}, allowing to modify the LP parameters. Extract from \Cref{lst:configuration-full}, \Cref{lst-ln:rep-liq-param}}
    ]
mod BC-LP-MODEL-MODIFIERS is ---[\CodeLineBreak]
--- operator used to insert a new `LiqParams` object    
op addLiqParams(_,_,_) : Configuration Float0+  
                         Float0+ ->          
                            Configuration .  
--- equation inserting the new object                         
eq addLiqParams(gamma, cminV, rliqV) = 
      gamma < P(0) : LiqParams | CMin(cminV), 
                                 Rliq(rliqV) > .
--- operator wrapping the `Configuration` into a
--- `closedConfiguration`
op addLiqParams(_,_,_) : closedConfiguration Float0+
                         Float0+ -> 
                               closedConfiguration .
eq addLiqParams(cGamma, cminV, rliqV) = 
     [ addLiqParams((cGamma).config, cminV, rliqV) ] .

--- operator updating `CMin` and `Rliq` values
op (_).replaceLiqParams(_,_) : closedConfiguration ---[\label{lst-ln:repLiqP}]
                             Float0+ Float0+
                             -> closedConfiguration .
eq (cGamma).replaceLiqParams(cminV, rliqV) = 
   [ ((cGamma).config).$replaceLiqParams(none, 
                                         cminV, rliqV) ] .
op (_).$replaceLiqParams(_,_,_) : Configuration 
                                  Configuration
                                  Float0+ Float0+
                                    -> Configuration .
eq (none).$replaceLiqParams(gamma', cminV, rliqV) = ---[\label{lst-ln:liqParams-add}]
          addLiqParams(gamma', cminV, rliqV) .
eq (gamma < P(0) : LiqParams | attrS >)  ---[\label{lst-ln:liqParams-upd}]
            .$replaceLiqParams(gamma', cminV, rliqV) = 
gamma < P(0) : LiqParams | CMin(cminV), 
                           Rliq(rliqV) > gamma' . ---[\CodeLineBreak]
endfm
\end{lstlisting}
\end{mdframed}

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=-3.6\baselineskip]
  \begin{lstlisting}[
    style=maude-snippet-style,
    label=lst:liq-params-destr,
    caption={Maude definition of the operators used to access \texttt{CMin} and \texttt{Rliq} values in a given configuration \texttt{gamma}. Extract from \Cref{lst:configuration-full}, \Cref{lst-ln:liq-param-destr}}
    ]
mod BC-LP-CONFIGURATION is ---[\CodeLineBreak]
--- assumes there is only one LiqParams object in gamma
op (_).params : Configuration -> [Configuration] .
eq (gamma).params = $params(gamma) . 
--- The auxiliary operator $params, returning the LiqParams 
--- object in gamma, is omitted ---[\CodeLineBreak]

op (_).CMin : Configuration -> Float0+ . 
eq (gamma).CMin = ((gamma).params).CMin .

op (_).Rliq : Configuration -> Float0+ .
eq (gamma).Rliq = ((gamma).params).Rliq . ---[\CodeLineBreak]
endfm
\end{lstlisting}
\end{mdframed}


\SSecSSSec{Validation of the LP specifications}
\label{subsec:test}

% 0. Tests form (unit vs integration)
% 1. Give an example

The standard Maude command \texttt{reduce} is employed to unit-test the specifications. The \texttt{reduce} command (abbreviated by \texttt{red}) reduces input terms into their corresponding canonical form terms, by progressively applying equational simplification steps, as detailed in \Cref{subsec:fmod}. The deterministic behaviour of reduce makes it a suitable command to test the specifications. In order to make the tests results immediately verifiable, the test cases were designed so that they would always return a boolean literal that equals to true if and only if the test case passes. \Cref{lst:unit-test} shows an example of a set of unit tests for a simple operator defined over agents' wallets, their semantics is indicated in the comments above each test. 

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=\MListFrm\baselineskip]
  \begin{lstlisting}[
    style=maude-syntax-def-style,    
    label=lst:unit-test,
    caption={Unit-test of the operator summing a \texttt{Token} to \texttt{Float0+} with a \texttt{Token} \texttt{Float0+} pair, as defined in \Cref{lst:wallet-full}, \Cref{lst-ln:sum-map-val-tok}.}
    ]
--- If the token type of the added value is not in the map
--- -> a new entry is added
red in WALLET : (tau(0) |-> 1.0) + 5.0 : tau(1)  == 
                 ((tau(0) |-> 1.0) ; (tau(1) |-> 5.0)) .

--- If the token type in map -> token amount is summed up
red in WALLET : (tau(0) |-> 1.0) + 5.0 : tau(0)  == 
                 (tau(0) |-> 6.0) .

--- If the map comprises multiple entries -> sum the
--- the value of the right token type                  
red in WALLET : ((tau(0) |-> 1.0) ; (tau(1) |-> 1.0)) + 
                             5.0 : tau(0) == 
                  (tau(0) |-> 6.0) ; (tau(1) |-> 1.0) .
\end{lstlisting}
\end{mdframed}

Conversely, the more advanced \texttt{search} command is utilised to perform "integration-tests" on the rewriting rules of the specifications. In fact, \texttt{search} is capable of exploring the entire state space reachable by applying a finite number of rewriting rules, as explained in \Cref{subsec:reach-analysis}. These test cases could not be designed so to return boolean values, as they test properties on multiple configurations. Thus, they appear less immediate to verify than the aforementioned tests. However, they are still very convenient to test interactions between the model components. \Cref{lst:integration-test} illustrates an integration test for the rule modelling the heuristic which powers rational liquidators, discussed in \Cref{chap:agents}. 

Totally, more than 350 tests have been developed in order to validate the specification of the LP model. For brevity, tests have not been included in the Appendices. However, they are available in the project repository \cite{mirelli2021maudelp}.

\begin{mdframed}[style=codeframe-style,
                 innerbottommargin=-3.6\baselineskip]
  \begin{lstlisting}[
    style=maude-syntax-def-style,    
    label=lst:integration-test,
    caption={Integration test of the liquidator agent behaviour, in scenario when borrower collateralization is less than \texttt{Rliq}. The tested rule is defined in \Cref{lst:agents-full}, \Cref{lst-ln:issue-liquidate}.}
    ]
--- This checks the number of all canonical final states,
--- which is 7.
search in LIQUIDATOR-TEST :
   (test12) =>! X:closedConfiguration .
--- Number of canonical final states satisfying the where
--- LED(0)'s collateralization is 0.0, then
--- expected = 7 
search in LIQUIDATOR-TEST :
   (test12) =>! X:closedConfiguration
   such that 
        ((X:closedConfiguration).config).C(LED(0)) == 0.0  .
\end{lstlisting}
\end{mdframed}




==> Chapters/7-conclusions.tex <==
\chapter{Conclusions}
\label{chap:conclusions}

% You have done your work, but that's\footnote{By the way, do \emph{not} use
% shorthands like this in your text! It is not professional! Always write out all
% the words: ``that is''.} not enough. 

% You also need to evaluate how well your implementation works.  The
% nature of the evaluation depends on your problem, your method, and
% your implementation that are all described in the thesis before this
% chapter.  If you have created a program for exact-text matching, then
% you measure how long it takes for your implementation to search for
% different patterns, and compare it against the implementation that was
% used before.  If you have designed a process for managing software
% projects, you perhaps interview people working with a waterfall-style
% management process, have them adapt your management process, and
% interview them again after they have worked with your process for some
% time. See what's changed.

% The important thing is that you can evaluate your success somehow.
% Remember that you do not have to succeed in making something spectacular; a
% total implementation failure may still give grounds for a very good master's
% thesis---if you can analyze what went wrong and what should have been
% done. 

 


==> Chapters/acronyms.tex <==

\ChapSecStar{Abbreviations and Acronyms}

% The longtable environment should break the table properly to multiple pages, if needed
\noindent
\begin{longtable}{@{}p{0.25\textwidth}p{0.7\textwidth}@{}}
  LP & Lending Pools \\
  DeFi & Decentralised Finance \\    
  LFM & Loanable Funds Markets \\ 
  TTP & Trusted Third Party \\
  DLT & Distributed Ledgers Technologies \\
  GBM & Geometric Brownian Motion \\
  LTL & Linear Temporal Logic \\
  SMC & Statistical Model Checking \\
  GNU & GNU's Not Unix! \\        
  GPL & General Public License \\
  % CI & Confidence Interval \\  
\end{longtable}


==> Chapters/appendices.tex <==
%\section{Maude specifications}
%\label{chapter:app-maude}
%
%\SecSubSec{Abstract datatypes}
%
%This listing specifies the main abstract data types, utilised in the rest of the LP model specifications. The main specified modules are:
%
%\begin{tabularx}{1.0\linewidth}{l X}
%  \RSep
%  \texttt{SUBSET} & specifies sets of tokens types;
%  \RSep                    
%  \texttt{MAP}    & models maps (or dictionaries) in Maude and  it is mainly defined accordingly to the native Maude library \texttt{prelude.maude}, as later discussed;
%  \RSep                                      
%  \texttt{MAP-TH} & implements functions (in the mathematical sense), binding target sorts to the ones in \texttt{FUNCTION};
%  \RSep
%  \texttt{FUNCTION} & implements functions (in the mathematical sense), containing the logic for computing domain and codomain;
%  \RSep
%  \texttt{HO-FILTER} & implements the filtering using higher order functions.
%  \RSep
%\end{tabularx}
%
%The fundamental difference between \texttt{Map\{X,Y\}} used in LP specification and the original is shown in \Cref{lst:prel-map-ctor}, illustrating the declaration of the original \texttt{Map\{X,Y\}}'s constructor. Notably, this operator differs than the LP one, \Cref{lst:abs-full} \Cref{lst-ln:lp-map-ctor}, for the two reasons detailed below.
%
%\begin{enumerate}
%  \item The former constructs a \texttt{Map} from \texttt{Map} terms only, whereas the latter constructs a \texttt{Map} term incrementally from \texttt{Entr}ies.
%  \item The former does not utilise kinds, while the latter does.
%\end{enumerate}
%
%These modifications to the original \texttt{Map} have been made, in order to develop the type system of tokens' \texttt{Map}s, which is not discussed in this thesis. 
%
%\begin{mdframed}[style=codeframe-style,
%                 innerbottommargin=\MListFrm\baselineskip]
%  \begin{lstlisting}[
%    style=maude-syntax-def-style,    
%    label=lst:prel-map-ctor,
%    caption={Maude original definition of \texttt{Map\{X,Y\}}, as per \texttt{prelude.maude}.}
%    ]
%op _,_ : Map{X,Y} Map{X,Y} -> Map{X,Y} 
%   [ctor assoc comm id: empty prec 121 format (d r os d)] .
%   \end{lstlisting}
%\end{mdframed}
%
%
%\begin{mdframed}[style=codeframe-style,
%                 innerbottommargin=\MListFrm\baselineskip]
%  \lstinputlisting[
%  linerange={ 
%    98-116,  % SUBSET
%    172-217, % MAP
%    229-247, % MAP-TH
%    285-349  % SUBMAP
%             % FUNCTION 
%    },       % HO-FILTER
%  %%consecutivenumbers=false,  
%  style=maude-file-style,
%  language=maude,
%  caption={\texttt{abstract-datatypes.maude} - Maude specifications of parameterised data types},  
%  label=lst:abs-full,
%  ]{../model/abstract-datatypes.maude}
%\end{mdframed}
%
%\SecSubSec{Tokens}
%
%This listing specifies the sorts and operators implementing token types and sets of token types.
%
%\begin{mdframed}[style=codeframe-style,]
%  \lstinputlisting[
%  % linerange={1-10,20-30,40-50},
%  % %consecutivenumbers=false,
%  style=maude-file-style,
%  language=maude,
%  caption={\texttt{tokens.maude} - Maude specifications of tokens},  
%  label=lst:tokens-full,
%  ]{../model/tokens.maude}
%\end{mdframed}
%
%\SecSubSec{Wallets}
%
%This listing specifies the sorts and operators implementing the wallets function $\Wallet$. The main specified modules are:
%
%\begin{tabularx}{1.0\linewidth}{l X}
%  \RSep
%  \texttt{WALLET} & defines the syntax and APIs offered by the wallets function, $\Wallet$;
%  \RSep                    
%  \texttt{PI-FUND} & defines the syntax and APIs offered by $\PoolFunds$.
%  \VSkip \\ \hline
%\end{tabularx}
%
%\begin{mdframed}[style=codeframe-style,
%                 innerbottommargin=\MListFrm\baselineskip]
%  % insert more lines if needed
%  \lstinputlisting[
%  linerange={piFund}, % PI-FUND
%  %consecutivenumbers=false,
%  style=maude-file-style,
%  language=maude,
%  caption={\texttt{wallets.maude} - Maude specifications of agent wallets and $\pi_{f}$},
%  label=lst:wallet-full,
%  ]{../model/wallets.maude}
%\end{mdframed}
%
%\SecSubSec{Pools}
%
%This listing specifies the sorts and operators implementing the pool object $\Pool$. The main specified modules are:
%
%\begin{tabularx}{1.0\linewidth}{l X}
%  \RSep
%  \texttt{LP}    & defines the services offered by a pool $\Pool$;
%  \RSep
%  \texttt{BC\{LP\}} & defines the syntax of an LP state, comprising a pool $\Pool$ and a price function $\Price$.
%  \VSkip \\ \hline
%\end{tabularx}
%
%\begin{mdframed}[style=codeframe-style,
%                 innerbottommargin=\MListFrm\baselineskip]
%  \lstinputlisting[
%  linerange={ 
%    lp,     % LP
%    bcLp}, % BC{LP}
%  %consecutivenumbers=false,
%  style=maude-file-style,
%  language=maude,
%  caption={\texttt{pools.maude} - Maude specifications of LPs main data structure: $\pi$},  
%  label=lst:pools-full,
%  ]{../model/pools.maude}
%\end{mdframed}
%
%\SecSubSec{Configurations}
%
%This listing specifies the sorts and operators implementing a lending pool configuration $\ConfObj$. The main specified modules are:
%
%\begin{tabularx}{1.0\linewidth}{l X}
%  \RSep  
%  \texttt{CONFIGURATION} & models a generic Maude configuration and it is mainly defined accordingly to the native Maude library \texttt{prelude.maude}, as later discussed;
%  \RSep                             
%  \texttt{LP-PARAMETERS} & defines the LP parameters $\CMin$, $\Rliq$ and $\Maxliq$;
%  \RSep                                                      
%  \texttt{BC-LP-MODEL}   & defines the LP rules;
%  \RSep                                                      
%  \texttt{BC-LP-MOD-MOD} & defines extra services for an LP configuration, used for the integration with MultiVeStA.  
%  \VSkip \\ \hline
%\end{tabularx}
%
%% In Maude, kinds specify error terms (also called ill-formed terms) of a sentence in the defined language.
%It is essential to note that Maude provides the implementation for a generic \texttt{Configuration}\footnote{Introduced in \Cref{subsec:mod}.}. However,  the LP \texttt{Configuration} is slightly different and corresponds to the one shown in \Cref{lst:conf-def,lst:configuration-full}, \Cref{lst-ln:configuration}. \Cref{lst:conf-def-2} illustrates the original constructor for a \texttt{Configuration} multiset, which is the only remarkable difference with the LP \texttt{Configuration}, in \Cref{lst:configuration-full}, \Cref{lst-ln:config-ctor}. As it is evident, the change only affects the operator input sorts, being \texttt{[Configuration]} in the operator used by LP specifications and \texttt{Configuration} in the original. This is motivated by the fact that \texttt{[Configuration]} identifies the kind of sort \texttt{Configuration}. Consequently, the adopted operator allows to define well-formed terms for a \texttt{Configuration} by simply defining a conditional membership equation statement as the one shown in \Cref{lst:configuration-full}, \Cref{lst-ln:pi-uniqueness}. From the listing, a well-formed \texttt{Configuration} is defined to be one satisfying the condition \texttt{isLPStateUnique}. Intuitively, this function checks that only one term \texttt{(pi | p):BC\{LP\}} is contained in the input \texttt{Configuration}.
%
%\begin{mdframed}[style=codeframe-style,
%                 innerbottommargin=\MListFrm\baselineskip]
%  \begin{lstlisting}[
%    style=maude-syntax-def-style,    
%    label=lst:conf-def-2,
%    caption={Maude original definition of \texttt{Configuration}, as per \texttt{prelude.maude}.}
%    ]
%op __ : Configuration Configuration -> Configuration
%      [prec 53 ctor config assoc comm id: none] .
%  \end{lstlisting}
%\end{mdframed}
%
%% \begin{mdframed}[style=codeframe-style]
%%   \begin{lstlisting}[
%%     style=maude-syntax-def-style,    
%%     label=lst:mb-wf-conf,
%%     caption={Maude definition of a well-formed LP \texttt{Configuration}. Extract from \Cref{lst:configuration-full}, \Cref{lst-ln:pi-uniqueness}.}
%%     ]
%% --- LP State uniqueness check
%% cmb gamma : Configuration if isLPStateUnique(gamma, 0) == 1 .
%%   \end{lstlisting}
%% \end{mdframed}
%
%\begin{mdframed}[style=codeframe-style,
%                 innerbottommargin=\MListFrm\baselineskip]
%  % insert more lines if needed
%\lstinputlisting[
%  style=maude-file-style,
%  language=maude,
%  linerange={
%    1-43,          % -> CONFIGURATION
%    52-99,         % -> BC-LP-CONFIG-COMPONENTS
%    111-182,       % -> LP-PARAMETERS
%                   % max-liq-speed
%    201-335,       % -> BC-LP-CONFIGURATION    
%    811-813,       % BC-LP-MODEL
%    905-954,       % -> deposit
%    1179-1242,     % -> liquidate
%                   % -> transfer 
%    1756-1831      % -> updatePrice
%  },
%  %consecutivenumbers=false,
%  caption={\texttt{configurations.maude} - Maude specifications of an LP configuration},  
%  label=lst:configuration-full,
%  ]{../model/configurations.maude}
%\end{mdframed}
%
%\SecSubSec{Agents}
%
%This listing specifies the sorts and operators implementing the heuristic for a liquidator.
%
%\begin{mdframed}[style=codeframe-style,
%                 innerbottommargin=\MListFrm\baselineskip]
%  % insert more lines if needed
%  \lstinputlisting[
%  linerange={
%    selectLiqParams,
%    issueLiquidate
%  },
%  %consecutivenumbers=false,
%  style=maude-file-style,
%  language=maude,
%  caption={\texttt{agents.maude} - Maude specifications of the heuristic modelling a rational liquidator},  
%  label=lst:agents-full,
%  ]{../model/agents.maude}
%\end{mdframed}
%
%\SecSubSec{Integration with Maude LTL model checker}
%
%This listing specifies the sorts and operators implementing the integration with the Maude native LTL model checker, shipped in the library \texttt{model-checker.maude}.
%
%% 2-151  % -> lemma1
%
%\begin{mdframed}[style=codeframe-style,
%                 innerbottommargin=\MListFrm\baselineskip]
%  % insert more lines if needed
%  \lstinputlisting[
%  linerange={
%    lemma1
%       },
%  %consecutivenumbers=false,
%  style=maude-file-style,
%  language=maude,
%  caption={\texttt{ltl.maude} - Integration of the Maude specification with the \texttt{MODEL-CHECKER} module},  
%  label=lst:ltl-full,
%  ]{../model/ltl.maude}
%\end{mdframed}
%
%
%\clearpage

\section{Additional figures}
\label{chapter:add-figures}

\SecSubSec{Modelling stock prices}

\begin{figure}[H]
  \centering
  \begin{subfigure}[H]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{eth-hist.png}
    \caption{{\footnotesize 13/01/2018-14/04/2018}}
    \label{fig:eth-hist}
  \end{subfigure}
% \end{figure}
% \begin{figure} \ContinuedFloat
%   \centering
  \medskip
  \begin{subfigure}[H]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{usdc-hist.png}
    \caption{{\footnotesize 01/01/2020-01/04/2020}}
    \label{fig:usdc-hist}
  \end{subfigure}
  \medskip       
  \begin{subfigure}[H]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{wbtc-hist.png}
    \caption{{\footnotesize 24/11/2020-23/02/2021}}
    \label{fig:wbtc-hist}
  \end{subfigure}
  \caption{Distributions of daily log returns computed from trimester closing prices}
  \label{fig:log-ret-hist}
\end{figure}

\begin{figure}[H]
  \centering
  \begin{subfigure}[H]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{collateral-eth-wbtc.png}
    \caption{}    
    % \caption{Predictions based on GBM instantiated with ETH parameters, in prices model scenario eth-wbtc.}
    \label{fig:unnorm-coll-eth-wbtc}
  \end{subfigure}
  \medskip       
  \begin{subfigure}[H]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{collateral-eth-usdc.png}
    \caption{}
    % \caption{Predictions based on GBM instantiated with ETH parameters, in prices model scenario eth-usdc.}
    \label{fig:unnorm-coll-eth-usdc}
  \end{subfigure}
  \medskip
  % \end{figure}
  % \begin{figure}[h] \ContinuedFloat
  %   \centering
  \begin{subfigure}[H]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{collateral-usdc-wbtc.png}
    \caption{}    
    % \caption{Predictions based on GBM instantiated with USDC parameters, in prices model scenario usdc-wbtc.}         
    \label{fig:unnorm-coll-usdc-wbtc}
  \end{subfigure}
  \caption{Prices predictions for the collateral assets produced, for each scenario in \Cref{tab:prices-pairs}, by GBMs instantiated with the parameters in \Cref{tab:gbm-params}.}
  \label{fig:unnorm-coll-all}
\end{figure}

\begin{figure}[H]
  \centering
  \begin{subfigure}[H]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{loan-eth-wbtc.png}
    \caption{}    
    % \caption{Predictions based on GBM instantiated with WBTC parameters, in prices model scenario eth-wbtc.}
    \label{fig:unnorm-loan-eth-wbtc}
  \end{subfigure}
  \medskip       
  \begin{subfigure}[H]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{loan-eth-usdc.png}
    \caption{}    
    % \caption{Predictions based on GBM instantiated with USDC parameters, in prices model scenario eth-usdc.}
    \label{fig:unnorm-loan-eth-usdc}
  \end{subfigure}
  \medskip
  % \end{figure}
  % \begin{figure}[h] \ContinuedFloat
  %   \centering
  \begin{subfigure}[H]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{loan-usdc-wbtc.png}
    \caption{}    
    % \caption{Predictions based on GBM instantiated with WBTC parameters, in prices model scenario usdc-wbtc.}         
    \label{fig:unnorm-loan-usdc-wbtc}
  \end{subfigure}
  \caption{Prices predictions for the loan assets produced, for each scenario in \Cref{tab:prices-pairs}, by GBMs instantiated with the parameters in \Cref{tab:gbm-params}.}
  \label{fig:unnorm-loan-all}
\end{figure}

\SecSubSec{Results of the statistical analysis}

\begin{figure}[H]
  \centering
  \includegraphics[scale=0.5,angle=90]{n-sims.png}
  \caption{Number of LP simulations, per \texttt{CMin-rliq} choices, performed to obtain an acceptable approximation of the per-agent collateralization (\Cref{fig:3d-1-5,fig:3d-3-7,fig:3d-all}).}
  \label{fig:n-sims}
\end{figure}

\begin{figure}[H]
  \centering
  \begin{subfigure}[H]{\textwidth}
    \centering
    \includegraphics[angle=90]{s-eth-wbtc-cmin-rliq-ag_1_10.png}
    \caption{Scenario: eth-wbtc.}
    \label{fig:s-eth-wbtc-cmin-rliq-ag_1_10}
  \end{subfigure}
\end{figure}
\begin{figure} \ContinuedFloat
  \centering
  % \medskip
  \begin{subfigure}[H]{\textwidth}
    \centering
    \includegraphics[angle=90]{s-eth-usdc-cmin-rliq-ag_1_10.png}
    \caption{Scenario: eth-usdc.}
    \label{fig:s-eth-usdc-cmin-rliq-ag_1_10}
  \end{subfigure}
  % \medskip 
\end{figure}
\begin{figure} \ContinuedFloat
  \begin{subfigure}[H]{\textwidth}
    \centering
    \includegraphics[angle=90]{s-usdc-wbtc-cmin-rliq-ag_1_10.png}
    \caption{Scenario: usdc-wbtc.}
    \label{fig:s-usdc-wbtc-cmin-rliq-ag_1_10}
  \end{subfigure}
  \caption{Per-borrower collateralization in the three prices scenarios, with varying liquidation rounds and \texttt{CMin-rliq} choices.}
  \label{fig:3d-all}
\end{figure}

\clearpage

%\section{Lending pools simulation}
%
%\SecSubSec{Full running example}
%
%\begin{mdframed}[style=codeframe-style,
%                 innerbottommargin=\MListFrm\baselineskip]
%  \lstinputlisting[
%  %consecutivenumbers=false,  
%  style=maude-file-style,
%  language=maude,
%  caption={\texttt{search.maude} - Full running example representing the configurations in \Cref{tab:run-ex}},  
%  label=lst:search-run-ex-full,
%  ]{../model/results/search.maude}
%\end{mdframed}
%




==> figures/general-star-graphs.tex <==
\begin{tikzpicture}[x=\graphgridsize,y=\graphgridsize] 

\coordinate (o) at (0,0);
\fill[black] (o) circle (\graphdotsize);
\foreach \d in {0, 90, ..., 270} {
  \coordinate (tmp) at ($(o) + (\d:1.5)$);
  \draw (o) -- (tmp);
  \fill[black] (tmp) circle (\graphdotsize);
}

\coordinate[right=4 of o] (o);
\coordinate (o1) at ($(o) + (0:0.3)$);
\coordinate (o2) at ($(o) + (180:0.3)$);
\fill[black] (o1) circle (\graphdotsize);
\fill[black] (o2) circle (\graphdotsize);
\draw (o1) -- (o2);
\foreach \d in {45, 135, 270} {
  \coordinate (tmp\d) at ($(o) + (\d:1.5)$);
  \draw (o2) -- (tmp\d);
  \fill[black] (tmp\d) circle (\graphdotsize);
}
\draw (o1) -- (tmp45);


\coordinate[right=4 of o] (o);
\coordinate (o1) at ($(o) + (0:0.3)$);
\coordinate (o2) at ($(o) + (180:0.3)$);
\fill[black] (o1) circle (\graphdotsize);
\fill[black] (o2) circle (\graphdotsize);
\draw (o1) -- (o2);
\foreach \d in {45, 135, 270} {
  \coordinate (tmp\d) at ($(o) + (\d:1.5)$);
  \draw (o2) -- (tmp\d);
  \fill[black] (tmp\d) circle (\graphdotsize);
}
\draw (o1) -- (tmp45);
\draw (o1) -- (tmp135);


\coordinate[right=4 of o] (o);
\coordinate (o1) at ($(o) + (0:0.3)$);
\coordinate (o2) at ($(o) + (180:0.3)$);
\fill[black] (o1) circle (\graphdotsize);
\fill[black] (o2) circle (\graphdotsize);
\draw (o1) -- (o2);
\foreach \d in {45, 135, 270} {
  \coordinate (tmp\d) at ($(o) + (\d:1.5)$);
  \draw (o1) -- (tmp\d);
  \draw (o2) -- (tmp\d);
  \fill[black] (tmp\d) circle (\graphdotsize);
}


\coordinate[right=3.5 of o] (o);
\coordinate (o1) at ($(o) + (90:0.3)$);
\coordinate (o2) at ($(o) + (210:0.5)$);
\coordinate (o3) at ($(o) + (330:0.5)$);
\fill[black] (o1) circle (\graphdotsize);
\fill[black] (o2) circle (\graphdotsize);
\fill[black] (o3) circle (\graphdotsize);
\draw (o1) -- (o2);
\draw (o1) -- (o3);
\draw (o2) -- (o3);
\foreach \d in {90, 270} {
  \coordinate (tmp\d) at ($(o) + (\d:1.5)$);
  \draw (o2) -- (tmp\d);
  \draw (o3) -- (tmp\d);
  \fill[black] (tmp\d) circle (\graphdotsize);
}
\draw (o1) -- (tmp90);


\coordinate[right=3 of o] (o);
\coordinate (o1) at ($(o) + (90:0.3)$);
\coordinate (o2) at ($(o) + (210:0.5)$);
\coordinate (o3) at ($(o) + (330:0.5)$);
\fill[black] (o1) circle (\graphdotsize);
\fill[black] (o2) circle (\graphdotsize);
\fill[black] (o3) circle (\graphdotsize);
\draw (o1) -- (o2);
\draw (o1) -- (o3);
\draw (o2) -- (o3);
\foreach \d in {90, 270} {
  \coordinate (tmp\d) at ($(o) + (\d:1.5)$);
  \draw (o2) -- (tmp\d);
  \draw (o3) -- (tmp\d);
  \fill[black] (tmp\d) circle (\graphdotsize);
}
\draw (o1) -- (tmp90);
\draw (o1) -- (tmp270);



\coordinate[right=3.5 of o] (o);
\coordinate (o1) at ($(o) + (18:1.3)$);
\coordinate (o2) at ($(o) + (90:1.3)$);
\coordinate (o3) at ($(o) + (162:1.3)$);
\coordinate (o4) at ($(o) + (234:1.3)$);
\coordinate (o5) at ($(o) + (306:1.3)$);
\foreach \d in {1, 2, ..., 5} {
  \fill[black] (o\d) circle (\graphdotsize);
}
\draw (o1) -- (o2);
\draw (o1) -- (o3);
\draw (o1) -- (o4);
\draw (o1) -- (o5);
\draw (o2) -- (o3);
\draw (o2) -- (o4);
\draw (o2) -- (o5);
\draw (o3) -- (o4);
\draw (o3) -- (o5);
\draw (o4) -- (o5);

\end{tikzpicture}


==> figures/obstruction-grouped.tex <==
\newlength{\oggs}
\setlength{\oggs}{1.2\graphgridsize}
\begin{tikzpicture}[x=\oggs,y=\oggs,every pin edge/.style={draw,dotted},pin distance=0.5\oggs,area/.style={ellipse,draw,dashed}] 

% The graph (0,0,5,0)
% o = origo
\coordinate (o) at (0,0);
\coordinate[left=1 of o,pin=100:$q_1$] (q1);
\coordinate[right=1 of o,pin=80:$q_2$] (q2);
\fill[black] (q1) circle (\graphdotsize);
\fill[black] (q2) circle (\graphdotsize);
\foreach \d in {-2, -1, ..., 2} {
  \coordinate (tmp) at ($(o) + (0,\d)$);
  \draw (q1) -- (tmp);
  \draw (q2) -- (tmp);
  \fill[black] (tmp) circle (\graphdotsize);
}
\node[area,minimum height=5.3\oggs,minimum width=0.8\oggs,pin=94:$X_3$] at (o) {};  

% The graph (1,0,3,0)
\coordinate[right=5 of o] (o);
\coordinate[left=1 of o,pin=260:$q_1$] (q1);
\coordinate[left=2 of o] (q1v);
\coordinate[right=1 of o,pin=280:$q_2$] (q2);
\fill[black] (q1) circle (\graphdotsize);
\fill[black] (q2) circle (\graphdotsize);
\fill[black] (q1v) circle (\graphdotsize);
\draw (q1) -- (q1v);
\foreach \d in {-1, 0, 1} {
  \coordinate (tmp) at ($(o) + (0,\d)$);
  \draw (q1) -- (tmp);
  \draw (q2) -- (tmp);
  \fill[black] (tmp) circle (\graphdotsize);
}
\node[area,minimum height=3.3\oggs,minimum width=0.8\oggs,pin=266:$X_3$] at (o) {};  
\node[area,minimum height=0.8\oggs,minimum width=0.8\oggs,pin=260:$X_1$] at (q1v) {};  


% The graph (0,1,3,0)
\coordinate[right=4 of o] (o);
\coordinate[left=1 of o,pin=100:$q_1$] (q1);
\coordinate[right=1 of o,pin=80:$q_2$] (q2);
\coordinate[right=2 of o] (q2v);
\fill[black] (q1) circle (\graphdotsize);
\fill[black] (q2) circle (\graphdotsize);
\fill[black] (q2v) circle (\graphdotsize);
\draw (q2) -- (q2v);
\foreach \d in {-1, 0, 1} {
  \coordinate (tmp) at ($(o) + (0,\d)$);
  \draw (q1) -- (tmp);
  \draw (q2) -- (tmp);
  \fill[black] (tmp) circle (\graphdotsize);
}
\node[area,minimum height=3.3\oggs,minimum width=0.8\oggs,pin=94:$X_3$] at (o) {};  
\node[area,minimum height=0.8\oggs,minimum width=0.8\oggs,pin=80:$X_2$] at (q2v) {};  

% The graph (0,0,3,1)
\coordinate[right=5 of o] (o);
\coordinate[left=1 of o,pin=260:$q_1$] (q1);
\coordinate[right=1 of o,pin=290:$q_2$] (q2);
\fill[black] (q1) circle (\graphdotsize);
\fill[black] (q2) circle (\graphdotsize);
\draw (q1) -- (q2);
\foreach \d in {-1, 1, 2} {
  \coordinate (tmp) at ($(o) + (0,\d)$);
  \draw (q1) -- (tmp);
  \draw (q2) -- (tmp);
  \fill[black] (tmp) circle (\graphdotsize);
}
\node[area,minimum height=4.3\oggs,minimum width=0.8\oggs,pin=266:$X_3$] at ($(o) + (0,0.5)$) {};  

\end{tikzpicture}


==> figures/page-merge.tex <==
\newcommand*{\actver}{\smash{\ensuremath{v_{\text{\textit{active}}}}}}

\tikzstyle{lbl}=[font=\scriptsize,midway,sloped]
\tikzstyle{opendash}=[densely dotted,thick] 
\tikzstyle{opendeco}=[decoration={zigzag,amplitude=0.1em,segment length=0.6em}]
\tikzstyle{actverline}=[dashed]
\tikzstyle{entryline}=[densely dotted]
\tikzstyle{area}=[ellipse,draw,dashed]
\tikzstyle{liveentry}=[entryline,postaction={%
  decorate,%
  decoration={%
    markings,%
    mark=at position .5pt with{\arrowreversed[line width=.35pt]{|}};,
    mark=at position 1 with{%
      \arrow[line width=.8pt]{stealth}};%
  }%
}]
\tikzstyle{deadentry}=[entryline,postaction={%
  decorate,%
  decoration={%
    markings,%
    mark=at position .5pt with{\arrowreversed[line width=.35pt]{|}};,
    mark=at position 1 with{%
      \arrow[line width=.8pt]{stealth}};%
%      \arrow[line width=.35pt,black,fill=white]{*}};% 
  }%
}]
\tikzstyle{pageborder}=[thick]
\tikzstyle{pagename}=[anchor=center,text=black!50,font=\huge]
\newlength{\spexx}
\setlength{\spexx}{1.2cm}
\newlength{\spexy}
\setlength{\spexy}{.5cm}

\subfigure[Before]{
\begin{tikzpicture}[x=\spexx,y=\spexy,%
  every pin edge/.style={draw,dotted},%
  pin distance=.5\spexx]
  \small
  \coordinate (lo) at (0,-5);
  \coordinate (o) at (0,0);
  \coordinate (hi) at (0,7);
  \coordinate (loact) at (3,-5);
  \coordinate (oact) at (3,0);
  \coordinate (hiact) at (3,7);
  \coordinate (loinf) at (4,-5);
  \coordinate (oinf) at (4,0);
  \coordinate (hiinf) at (4,7);
  
  \draw[->] (lo) -- node[below,lbl] {Versions} ($(loinf) + (1em,0)$);
  \draw[->] (lo) -- node[above,lbl] {Keys} ($(hi) + (0,1em)$);

  \draw[pageborder] (lo) -- (o) -- (hi);
  \draw[pageborder] (lo) -- (loinf);
  \draw[pageborder] (hi) -- (hiinf);
  \draw[pageborder] (o) -- (oinf);

  \draw[opendash] decorate [opendeco] { (loinf) -- (oinf) };
  \draw[opendash] decorate [opendeco] { (oinf) -- (hiinf) };

  \node[pagename] at (2,3.5) {$p$};
  \node[pagename] at (2,-2.5) {$s$};

  \draw[actverline] ($(loact) + (0,-1em)$) node[below=.4em] {\actver} --
    ($(hiact) + (0,1em)$);

  % Page p contents
  \draw[deadentry] (0,6) -- (1,6);
  \draw[deadentry] (1,6) -- (2,6);
  \draw[deadentry] (2,6) -- (3,6);
  \draw[liveentry] (0,5) -- (4,5);
  \draw[deadentry] (0,4) -- (2,4);
  \draw[deadentry] (1,3) -- (3,3);
  \draw[deadentry] (0,2) -- (1,2);
  \draw[deadentry] (2,2) -- (3,2);
  \draw[deadentry] (0,1) -- (2,1);
  \draw[deadentry] (2,1) -- (3,1);

  % Page s contents
  \draw[liveentry] (0,-1) -- (4,-1);
  \draw[deadentry] (0,-2) -- (2,-2);
  \draw[deadentry] (0,-3) -- (3,-3);
  \draw[liveentry] (3,-4) -- (4,-4);

  \node[area,minimum width=4.5\spexx,minimum height=.6\spexy,pin=178:{$1$}]
    at (2,5) {};
  \node[area,minimum width=4.5\spexx,minimum height=.6\spexy,pin=182:{$2$}]
    at (2,-1) {};
  \node[area,minimum width=1.5\spexx,minimum height=.6\spexy,pin=330:{$3$}]
    at (3.5,-4) {};

\end{tikzpicture}}
\subfigure[After]{
\begin{tikzpicture}[x=\spexx,y=\spexy,%
  every pin edge/.style={draw,dotted},%
  pin distance=.5\spexx]
  \small
  \coordinate (lo) at (0,-5);
  \coordinate (o) at (0,0);
  \coordinate (hi) at (0,7);
  \coordinate (loact) at (3,-5);
  \coordinate (oact) at (3,0);
  \coordinate (hiact) at (3,7);
  \coordinate (loinf) at (4,-5);
  \coordinate (oinf) at (4,0);
  \coordinate (hiinf) at (4,7);

  \draw[->] (lo) -- node[lbl,below] {Versions} ($(loinf) + (1em,0)$);
  \draw[->] (lo) -- node[lbl,above] {Keys} ($(hi) + (0,1em)$);

  \draw[pageborder] (lo) -- (o) -- (hi);
  \draw[pageborder] (lo) -- (loinf);
  \draw[pageborder] (hi) -- (hiinf);
  \draw[pageborder] (o) -- (oact);

  \draw[opendash] decorate [opendeco] { (loinf) -- (oinf) };
  \draw[opendash] decorate [opendeco] { (oinf) -- (hiinf) };

  \node[pagename] at (1.5,3.5) {$p$};
  \node[pagename] at (1.5,-2.5) {$s$};
  \node[pagename] at (3.5,1) {$p'$};

  \draw[actverline] ($(loact) + (0,-1em)$) node[below=.4em] {\actver} -- (loact);
  \draw[pageborder] (loact) -- (hiact);
  \draw[actverline] (hiact) -- ($(hiact) + (0,1em)$);

  % Page p contents
  \draw[deadentry] (0,6) -- (1,6);
  \draw[deadentry] (1,6) -- (2,6);
  \draw[deadentry] (2,6) -- (3,6);
  \draw[deadentry] (0,5) -- (3,5);
  \draw[deadentry] (0,4) -- (2,4);
  \draw[deadentry] (1,3) -- (3,3);
  \draw[deadentry] (0,2) -- (1,2);
  \draw[deadentry] (2,2) -- (3,2);
  \draw[deadentry] (0,1) -- (2,1);
  \draw[deadentry] (2,1) -- (3,1);

  % Page s contents
  \draw[deadentry] (0,-1) -- (3,-1);
  \draw[deadentry] (0,-2) -- (2,-2);
  \draw[deadentry] (0,-3) -- (3,-3);

  % Page p' contents
  \draw[liveentry] (3,5) -- (4,5);
  \draw[liveentry] (3,-1) -- (4,-1);
  \draw[liveentry] (3,-4) -- (4,-4);

  \node[area,minimum width=1.5\spexx,minimum height=.6\spexy,pin=10:{$1$}]
    at (3.5,5) {};
  \node[area,minimum width=1.5\spexx,minimum height=.6\spexy,pin=3:{$2$}]
    at (3.5,-1) {};
  \node[area,minimum width=1.5\spexx,minimum height=.6\spexy,pin=330:{$3$}]
    at (3.5,-4) {};
\end{tikzpicture}}

